Masked Language Modeling and the Distributional Hypothesis: Order Word Matters Pre-training for Little

A possible explanation for the impressive performance of masked language model (MLM) pre-training is that such models have learned to represent the syntactic structures prevalent in classical NLP pipelines. In this paper, we propose a different explanation: MLMs succeed on downstream tasks almost entirely due to their ability to model higher-order word co-occurrence statistics. To demonstrate this, we pre-train MLMs on sentences with randomly shuffled word order, and show that these models still achieve high accuracy after fine-tuning on many downstream tasks -- including on tasks specifically designed to be challenging for models that ignore word order. Our models perform surprisingly well according to some parametric syntactic probes, indicating possible deficiencies in how we test representations for syntactic information. Overall, our results show that purely distributional information largely explains the success of pre-training, and underscore the importance of curating challenging evaluation datasets that require deeper linguistic knowledge.

==> sections/intro.tex <==
Our field has become dominated by the pretrain-and-finetune paradigm, where we first obtain a good parametric \emph{prior} in order to subsequently efficiently model downstream tasks. In its recent masked language model (MLM) pretraining incarnation, as epitomized by BERT, this approach has proven wildly successful. BERT, of course, builds on solid foundations that span back decades [citeLSAWestonMikolov], in that it exploits the well-known distributional hypothesis [citeHarris]. One might even argue that BERT, despite all its merits, is not actually all that different from earlier distributional models like word2vec [citeMikolov]~(see Appendix A). On the other hand, it has been claimed that BERT ``rediscovers the classical NLP pipeline'', suggesting that it has learned ``the kind of abstractions that we intuitively believe are important for representing natural language'' rather than ``simply modeling complex co-occurrence statistics'' [citeTenney].

In this work, we try to uncover how much of MLM's performance comes from simple distributional information, as opposed to ``the types of syntactic and semantic abstractions traditionally believed necessary for language processing'' [citeTenney]. For the latter, which is admittedly not very well-defined, we take the \emph{word order} of a sentence as the primary and most straightforward proxy: presumably, any sophisticated NLP pipeline depends on the important syntactic information conveyed by the order of words. Surprisingly, we find that most of MLM's high performance can in fact be explained by the ``distributional prior'' rather than its ability to substitute for the classical NLP pipeline.

Concretely, we pretrain MLM (RoBERTa [cite]) models on randomized data with permuted word order and examine their downstream performance. We establish a baseline on a corpus sampled from the source corpus' unigram probability distribution. We then train models on various degrees of permuted data that preserve sentence-level distributional information, by randomly shuffling $n$-grams within the sentence where $n \in {1,2,3,4}$. We also experiment with training MLM transformers with removed positional embeddings, making them order agnostic. These permuted models are evaluated in a wide range of settings and compared against standard regularly-pretrained models. 

We demonstrate that pretraining on permuted data has surprisingly little effect on downstream task performance. This is partially explained by inductive biases that are present in the model itself, as illustrated by the baseline model performing reasonably well. That model is vastly outperformed, however, by permuted models where sentence-level distributional information was preserved. It has recently been found that MLM models are quite robust to permuting downstream test data [cite] and even do reasonably well on permuted ``unnatural'' downstream train data [cite]. To the best of our knowledge, this work is the first to show that downstream performance for ``unnatural language pretraining'' is much closer to standard MLM than we might have expected.

In an effort to shed light on these findings, we experiment with various probing tasks. We verify via non-parametric probes that the permutations do in fact make the model much worse at syntax-dependent tasks. However, just like on the downstream tasks, permuted order-agnostic models perform very well on parametric syntactic probes, almost matching the unpermuted model's performance, which is quite surprising given how important order is for syntax. This again suggests that BERT's success in downstream tasks is mostly explained by it having learned higher-order distributional statistics that make for a useful prior.

Depending on your position in NLP's great debates, you might draw different conclusions from these findings. One might argue that our downstream tasks are flawed evaluations, and that we need to examine models with examples that truly test strong generalization and compositionality. Alternatively, one could argue that human language understanding might similarly depend on the structure (i.e., order) of the \emph{world} for a large or even the most part. Or perhaps we are just not focusing enough on the tail of the distribution, where true syntactic capabilities would certainly be borne out. While these results are somewhat disappointing for NLP at large, this work also offers a message of hope and sense of purpose: can we design tasks that require more sophisticated reasoning, true compositionality, robustness against adversaries and strong human-like generalization? Can we design better experimental protocols for testing the phenomena we really care about? Can we be more careful with our baselines? The purpose of this work is to put our understanding of MLM pretraining on more solid footing, and we hope to inspire future work in these important directions.

%%% Previous intro ending
Our contributions:

\begin{itemize}
    \item We find permuting word-order while pre-training to have surprisingly low effect on downstream tasks (GLUE, PAWS).
    \item We observe majority of word-order information models acquire is learned during fine-tuning, with some tasks being more sensitive than others.
    \item We observe that non-parametric measures are much better at distinguishing pre-trained models trained on permuted word-order than parametric probing tasks.
\end{itemize}


==> tables/glue.tex <==
\begin{table*}[t]
  \centering
  \resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lrrrrrrrl}
\toprule
Model &  QNLI &   RTE &   QQP &  SST-2 &  MRPC &  CoLA &  PAWS &           MNLI (m/mm) \\
\midrule
   OR & 0.925 & 0.746 & 0.913 &  0.939 & 0.892 & 0.614 & 0.945 &  0.861 / 0.854 \\
   R1 & 0.890 & 0.690 & 0.910 &  0.905 & 0.860 & 0.352 & 0.900 &  0.826 / 0.827 \\
   R2 & 0.904 & 0.708 & 0.914 &  0.918 & 0.862 & 0.544 & 0.935 &  0.834 / 0.835 \\
   R3 & 0.917 & 0.707 & 0.912 &  0.920 & 0.864 & 0.487 & 0.940 &  0.838 / 0.838 \\
   R4 & 0.917 & 0.708 & 0.914 &  0.925 & 0.870 & 0.587 & 0.943 &  0.838 / 0.839 \\ \hline
   RC & 0.711 & 0.540 & 0.855 &  0.834 & 0.705 & 0.000 & 0.585 &  0.719 / 0.715 \\
\bottomrule
\end{tabular}}
\caption{GLUE and PAWS dev set results on RoBERTa (base), trained on variants of BookWiki corpus. We use the same evaluation setup of \citet{liu2019b}, and report the median over 5 seeds for the best hyperparam configuration.}
\label{table:glue}
\end{table*}


==> tables/gulordava.tex <==
\begin{table*}
  \centering
  \resizebox{\linewidth}{!}{%
\begin{tabular}{lllllll}
\toprule
Model &               \OR &               \RI &               \RII &               \RIII &               \RIV &               \RC \\
Condition &               &               &               &               &               &               \\
\midrule
0         &  72.22 (2.4e+00) &  42.84 (3.2e-02) &  52.46 (4.8e-02) &  55.56 (1.4e-01) &  56.94 (1.7e-01) &  35.26 (-1.4e-04) \\
1         &  77.08 (2.5e+00) &  76.56 (1.9e-02) &  72.4 (-8.9e-02) &  71.88 (2.1e-01) &  71.35 (6.1e-01) &   59.38 (9.5e-04) \\
2         &  55.56 (9.2e-01) &  81.48 (3.1e-02) &  51.85 (4.0e-02) &  62.96 (3.8e-01) &  74.07 (6.1e-01) &   77.78 (2.7e-04) \\
\bottomrule
\end{tabular}}
\caption{\citet{gulordava2018} stimuli results in raw accuracy. Values in parenthesis reflect the $P(\textrm{good}) - P(\textrm{bad})$ metric.}
\label{tab:gul_full}
\end{table*}


==> tables/marvin_linzen.tex <==
\begin{table*}
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lllllll}
\toprule
Model &               \OR &               \RI &               \RII &               \RIII &               \RIV &               \RC \\
Condition &                  &                   &                  &                  &                  &                  \\
\midrule
AOR       &  90.02 (2.9e+01) &   60.36 (1.7e+00) &  66.45 (3.9e+00) &  63.43 (2.5e+00) &  61.25 (1.2e+00) &   50.0 (4.2e-05) \\
AOR-T     &  77.34 (1.4e+01) &   78.94 (1.5e-01) &  52.24 (4.3e-01) &  48.87 (2.5e-01) &  56.62 (5.5e-01) &  50.0 (-1.9e-04) \\
APP       &  89.86 (2.7e+01) &   70.22 (6.8e-01) &  53.33 (2.0e-01) &  53.43 (7.9e-01) &  60.74 (9.1e-01) &  50.0 (-3.2e-03) \\
ARC       &   84.90 (1.2e+00) &   62.45 (1.1e-01) &  74.59 (7.0e-02) &  67.51 (6.7e-02) &  62.74 (3.4e-02) &  50.0 (-1.1e-05) \\
ASR       &  87.08 (2.6e+01) &   79.08 (1.9e+00) &  81.73 (2.9e+00) &  63.03 (1.4e+00) &  67.34 (1.5e+00) &  50.0 (-2.9e-03) \\
IOR       &  89.96 (4.0e-01) &   56.32 (6.2e-03) &  59.32 (3.8e-02) &  70.42 (4.1e-02) &  62.74 (8.4e-02) &  50.0 (-1.5e-03) \\
IOR-T     &  74.21 (2.0e-01) &   52.57 (6.2e-03) &   57.30 (1.3e-02) &  62.22 (6.2e-03) &  55.33 (2.7e-02) &  50.0 (-9.9e-04) \\
ISC       &  86.45 (5.3e+00) &   67.88 (6.7e-02) &  82.79 (4.8e-03) &  77.78 (3.1e-01) &   68.4 (5.9e-02) &   50.0 (3.1e-04) \\
LVC       &  93.58 (2.7e+01) &   70.42 (9.7e-02) &  87.75 (1.4e+00) &  85.25 (6.3e-01) &  81.42 (6.6e-01) &  50.0 (-3.3e-05) \\
SCM       &  88.66 (5.7e+00) &   63.31 (1.2e-01) &  82.27 (1.7e-01) &  86.67 (2.6e+00) &  80.07 (2.6e-01) &   50.0 (1.7e-02) \\
SNP       &  95.39 (2.3e-01) &  18.43 (-3.1e-03) &  51.76 (3.0e-03) &  77.51 (1.7e+00) &  53.93 (8.2e-02) &  50.0 (-3.1e-04) \\
SRX       &  89.88 (2.7e+00) &   87.38 (1.0e-01) &  91.07 (3.2e-01) &  94.29 (2.4e-02) &  91.43 (3.1e+00) &   50.0 (2.0e-04) \\
SVA       &  95.28 (3.1e+01) &   87.22 (5.7e-01) &  88.61 (3.2e+00) &  94.17 (6.1e+00) &  89.72 (3.1e+01) &   50.0 (2.2e-02) \\
SVC       &  97.45 (1.9e+01) &   82.82 (8.4e-01) &  83.94 (1.2e+00) &  92.64 (6.4e+00) &  80.74 (1.1e+01) &   50.0 (2.8e-04) \\
\bottomrule
\end{tabular}}
\caption{\citet{marvin-linzen-2018-targeted} stimuli results in raw accuracy. Values in parenthesis reflect the $P(\textrm{good}) - P(\textrm{bad})$ metric. Abbreviations: Simple Verb Agreement (SVA), In a sentential complement (SCM), Short VP Coordination (SVC), Long VP Coordination (LVC), Across a prepositional phrase (APP), Across a subject relative clause (ASR), Across an object relative clause (AOR), Across an object relative (no \textit{that}) (AOR-T),
    In an object relative clause (IOR),
    In an object relative clause (no \textit{that}) (IOR-T),
    Simple Reflexive (SRX), In a sentential complement (ISC),
    Across a relative clause (ARC), Simple NPI (SNP).}
\label{tab:marvin_full}
\end{table*}


==> tables/paws.tex <==
\begin{tabular}{lr}
\toprule
   name &      acc \\
\midrule
   orig & 0.944 \\
    n\_1 & 0.899 \\
    n\_2 & 0.934 \\
    n\_3 & 0.940 \\
    n\_4 & 0.943 \\
\bottomrule
\end{tabular}

==> tables/random_eval.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllllll}
\toprule
Model &           MRPC &            RTE &           PAWS &         SST-2 &           CoLA &           QNLI \\
\midrule
  \OR &  76.11 +/- 0.98 &  54.93 +/- 2.91 &  62.31 +/- 0.08 &  80.83 +/- 0.36 &   5.05 +/- 2.22 &  79.04 +/- 0.68 \\
  \RI &  81.24 +/- 1.28 &  65.53 +/- 3.57 &   62.63 +/- 0.1 &  83.84 +/- 0.35 &  23.42 +/- 6.49 &  87.29 +/- 0.17 \\
  \RII &   80.48 +/- 0.7 &  66.55 +/- 2.01 &  61.24 +/- 3.06 &  82.99 +/- 0.28 &   10.36 +/- 1.9 &  86.13 +/- 0.51 \\
  \RIII &  79.51 +/- 0.92 &  64.95 +/- 2.99 &  62.27 +/- 0.09 &    83.0 +/- 0.2 &    9.0 +/- 5.15 &  84.68 +/- 1.23 \\
  \RIV &  79.06 +/- 0.97 &  65.96 +/- 1.39 &  62.18 +/- 0.19 &  83.09 +/- 0.42 &   6.62 +/- 6.09 &  84.76 +/- 0.77 \\
\bottomrule
\end{tabular}}
\caption{Evaluation of the fine-tuned models on unigram randomized version of dev set for a subset of tasks in GLUE and PAWS.}
\label{tab:rand_eval}
\end{table}
